DeUEDroid: Detecting Underground Economy Apps Based on UTG Similarity

In recent years, the underground economy is proliferating in the mobile system. These underground economy apps (UEware) make profits from providing non-compliant services, especially in sensitive areas such as gambling, pornography, and loans. Unlike traditional malware, most of them (over 80%) do not have malicious payloads. Due to their unique characteristics, existing detection approaches cannot effectively and efficiently mitigate this emerging threat. To address this problem, we propose a novel approach to effectively and efficiently detect UEware by considering their UI transition graphs (UTGs). Based on the proposed approach, we design and implement a system named DeUEDroid to perform the detection. To evaluate DeUEDroid, we collect 25,717 apps and build the first large-scale ground-truth dataset (1,700 apps) of UEware. The evaluation result based on the ground-truth dataset shows that DeUEDroid can cover new UI features and statically construct precise UTG. It achieves 98.22% detection F1-score and 98.97% classification accuracy, significantly outperforming traditional approaches. The evaluation involving 24,017 apps demonstrates the effectiveness and efficiency of UEware detection in real-world scenarios. Furthermore, the result reveals that UEware are prevalent, with 54% of apps in the wild and 11% of apps in app stores being UEware. Our work sheds light on future work in analyzing and detecting UEware.

==> code/webview.tex <==
\lstset{
 columns=fixed,       
 %numbers=left,                                        % 在左侧显示行号
 numberstyle=\fontzise\color{gray},                       % 设定行号格式
 frame=none,                                          % 不显示背景边框
 backgroundcolor=\color[RGB]{245,245,244},            % 设定背景颜色
 keywordstyle=\color[RGB]{40,40,255},                 % 设定关键字颜色
 numberstyle=\footnotesize\color{darkgray},           
 commentstyle=\it\color[RGB]{0,96,96},                % 设置代码注释的格式
 stringstyle=\rmfamily\slshape\color[RGB]{128,0,0},   % 设置字符串格式
 showstringspaces=false,                              % 不显示字符串中的空格
 language=java,                                        % 设置语言
 breaklines = true, %% enable line breaking
 basewidth       =   0.5em
}
\begin{figure}[!t]
    \centering
\begin{lstlisting}
//Type-I: ImmediateBox Parameter
WebView.loadUrl("http://example.com");
//Type-II: Resource Parameter
WebView.loadUrl(this.getResources().getString(R.string.url));
//Type-III: Runtime Parameter
ReqeustURL = searchBox.getString();
WebView.loadUrl(ReqeustURL);
//Type-IV: Complex Parameter
ID.value = EditBox.getString();
url=this.getResources().getString(R.string.url)+"/?id="+ID.value()
WebView.loadUrl(url);
...
//res/values/string.xml
<resources> 
    <string name="url">http://example.com</string>
</resources>
\end{lstlisting}
    \caption{Three types of hybrid API Parameter}
    \label{fig:webview}
    \vspace{-1em}
\end{figure}

==> table/Hybrid.tex <==
\begin{table}[!tb]
\caption{The Common Hybrid Techniques.}
\centering
\footnotesize

\resizebox{.45\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
\multicolumn{3}{l}{{\color[HTML]{000000} Category}}   & {\color[HTML]{000000} Sub-Category} & Class Name \\
\midrule
\multicolumn{3}{l}{} & ImageLoader & com.nostra13.universalimageloader     \\
\multicolumn{3}{l}{} & Picasso & com.squareup.picasso.Picasso    \\
\multicolumn{3}{l}{} & Glide & com.bumptech.glide    \\
\multicolumn{3}{l}{\multirow{-4}{*}{Framework}} & Fresco & com.facebook.drawee     \\
\midrule

%\multicolumn{3}{l}{Okhttp3} & -& okhttp3.request  \\
%\midrule
\multicolumn{3}{l}{WebView} & - & android.webkit.WebView  \\
\bottomrule
\end{tabular}
}
\label{tab:webapi}
\vspace{-1em}
\end{table}

==> table/UEgroup.tex <==
\begin{table}[!tb]
    \centering
    %\resizebox{.45\textwidth}{!}{
    \begin{tabular}{c|c}
    \toprule
    \textbf{Underground Economy Scenario} & \textbf{Behavior} \\
    \midrule
      Gambling   & Apps offer a variety of entertainment activities/games (\eg, lotteries, gambling game) and lure victims to deposit \\
      \midrule
       Porn Trading  & 4 \\
       \midrule
       Financial Scam  & 4 \\
       \midrule
       Miscellaneous  & 4 \\
    \bottomrule
    \end{tabular}
    %}
    \caption{Underground Economy App Group}
    \label{tab:UEgroup}
\end{table}

==> table/WebView.tex <==
% \usepackage{multirow}

\begin{table}[!tb]
\centering
\resizebox{.4\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{llll}
\toprule
\multirow{2}{*}{\textbf{WebView Type}} & \multirow{2}{*}{\#} &  \multicolumn{2}{c}{Identified (\%)}  \\
\cmidrule{3-4} & & True & False  \\
\midrule
Type-I & 4 & 100\% & 0\% \\
Type-II & 5 & 100\% & 0\% \\
Type-III & 5 & 80\% & 20\% \\
Type-IV (with Type-III) & 3 & 0\% & 100\% \\
Type-IV (without Type-III) & 5 & 50\% & 50\% \\
\midrule
Total & 21 & 71.4\% & 28.8\% \\
\midrule
\end{tabular}
\end{threeparttable}
}
\caption{The Evaluation of WebView Recovery.}
\label{tab:static_eva_web}
\end{table}

==> table/thread.tex <==
\begin{table}[!tb]
\centering
\footnotesize

\resizebox{.45\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
\multicolumn{3}{l}{{\color[HTML]{000000} Top-Class Name}}   & {\color[HTML]{000000} Run Method} & Start Method \\
\midrule
\multicolumn{3}{l}{} & onPreExecute & execute     \\
\multicolumn{3}{l}{} & doInBackground & onPreExecute    \\
\multicolumn{3}{l}{\multirow{-3}{*}{AsyncTask}} & doPostExecute & doInBackground     \\
\midrule
\multicolumn{3}{l}{OnClickListener} & setOnClickListener & OnClick  \\
\midrule
\multicolumn{3}{l}{Runnable} & run & start  \\
\midrule
\multicolumn{3}{l}{Message} & handleMessage & sendMessage  \\
\bottomrule
\end{tabular}
}
\caption{The implicit run and start pairs.}
\label{tab:thread}
\vspace{-1em}
\end{table}
